GraphZero: Breaking Symmetry for Efficient Graph Mining

Graph mining for structural patterns is a fundamental task in many applications. Compilation-based graph mining systems, represented by AutoMine, generate specialized algorithms for the provided patterns and substantially outperform other systems. However, the generated code causes substantial computation redundancy and the compilation process incurs too much overhead to be used online, both due to the inherent symmetry in the structural patterns. In this paper, we propose an optimizing compiler, GraphZero, to completely address these limitations through symmetry breaking based on group theory. GraphZero implements three novel techniques. First, its schedule explorer efficiently prunes the schedule space without missing any high-performance schedule. Second, it automatically generates and enforces a set of restrictions to eliminate computation redundancy. Third, it generalizes orientation, a surprisingly effective optimization that was mainly used for clique patterns, to apply to arbitrary patterns. Evaluated on multiple graph mining applications and complex patterns with 7 real-world graph datasets, GraphZero demonstrates up to 40X performance improvement and up to 197X reduction on schedule generation overhead over AutoMine.

==> abstract.tex <==
%Something broke in the git when this was empty

==> algorithms/multiplicity_reduce_lazy.tex <==
\begin{algorithm}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\SetKwProg{procedure}{Procedure}{}{}
\DontPrintSemicolon
\Input{$ $ $P:$ the pattern.}
\Input{$ $ $S:$ the schedule.}
\Output{$ $ $restrictions:$ a map representing all chosen relations, implemented as an array. Unset values means there is no chosen relation}
\Begin{
    $Aut \gets$ all the automorphisms of $P$\\
    $restrictions\gets$ an empty mapping.\\
    \tcp{iterate through these in order, $S[0], S[1],\cdots$}
    \For{$V$ in  $S$}{
        \tcp{stabilized\_aut is the stabilized subgroup of the automorphism group, where all the vertices we have iterated over are fixed.}
        $stabilized\_ aut\gets []$\\
        \For{$x \in Aut$}{
            \If{$V^x= V$}{
                add $x$ to $stabilized\_aut$}
            \Else{
                %\tcp{Any schedule generated by $V^x$ as the first vertex is equivalent to one generated with $V$ as the first vertex, so we don't need to process it}
                set $restrictions[V^x] = V$}}
            $Aut\gets stabilized\_aut$}}
\caption{Restriction generation algorithm - lazy restrictions}
\label{alg:multiplicity_reduce_lazy}
\end{algorithm}


==> algorithms/schedule_reduced.tex <==
\begin{algorithm}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\SetKwProg{procedure}{Procedure}{}{}
\DontPrintSemicolon
\Input{$ $ $P:$ the pattern.}
\Output{$ $ $schedules:$ the list of all distinct valid schedules for $P$}
\Begin{
    $schedules\gets []$\\
    $Aut \gets$ all the automorphisms of $P$\\
    call recursive\_generate([],Aut)}
\procedure{recursive-generate}{    
    %\tcp{$V^x$, known as the action of $V$ under $x$, is what $x$ maps $V$ to}  
    \Input{sched - a partially built schedule}
    \Input{aut - all automorphisms on $P$ that do not move anything in sched}
    %\Output{None, just modifies the schedules list}
    %\tcp{aut is always a group - see stabilizer groups}
    %\tcp{The following iterates over all possible next vertices that would result in a valid schedule}
    \If{sched covers all vertices in the pattern}{add sched to schedules\\ End this procedure call}
    \For{Vertex $V\in P$ conn. to sched, not in sched}{
        \If{$V$ is marked as processed here}{
            continue from the start of the for loop}
        \Else{
            $stabilized\_aut\gets []$\\
            \For{$x \in Aut$}{
                \If{$V^x= V$}{
                    add $x$ to $stabilized\_aut$}
                \Else{
                 %\tcp{Any schedule generated by $V^x$ as the first vertex is equivalent to one generated with $V$ as the first vertex, so we don't need to process it}
                mark $V^x$ as processed here}}
            call recursive-generate(sched+[V],$stabilized\_aut$) }}}
\caption{Efficient Schedule generation algorithm}
\label{alg:sched_gen}
\end{algorithm}


==> algorithms/schedule_without_valid_next.tex <==
\begin{algorithm}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\SetKwProg{procedure}{Procedure}{}{}
\DontPrintSemicolon
\Input{$ $ $P:$ the pattern.}
\Output{$ $ $schedules:$ the list of all distinct valid schedules for $P$}
\Begin{
    $schedules\gets []$\\
    $Aut \gets$ all the automorphisms of $P$\\
    call recursive\_generate([],Aut, schedules)}
\procedure{recursive-generate}{    
    %\tcp{$V^x$, known as the action of $V$ under $x$, is what $x$ maps $V$ to}  
    \Input{sched - a partially built schedule}
    \Input{aut - automorphisms that move $v$ to $v$ for $v\in sched$}
    %\Input{relations - Binary relations that would be created in Algorithm~\ref{alg:multiplicity_reduce} that need to be enforced per Theorem~\ref{theorem:lazy_restrict}}
   \Input{schedules - list of distinct schedules}
    \If{sched covers all vertices in the pattern}{
    add $sched$ with partial ordering $relations$ to schedules\\
    End this procedure call}
    valid\_next$\gets$ vertices connected to $sched$ not in $sched$\\
    \For{$v\in valid\_next$ }{
        \If{$v$ is marked as processed}{
            continue}
        \Else{
            %relations\_copy$\gets relations$
            $stabilized\_aut\gets []$\\
            \For{$x \in Aut$}{
                \If{$x(v)= v$}{
                    add $x$ to $stabilized\_aut$}
                \Else{
                 %\tcp{Any schedule generated by $V^x$ as the first vertex is equivalent to one generated with $V$ as the first vertex, so we don't need to process it}
                mark $x(v)$ as processed\\
                %set $relations\_copy[x(v)]=v$
                }}
            call recursive-generate(sched+[v], $stabilized\_aut$,schedules)\\ }}}
\caption{Schedule generation algorithm }
\label{alg:sched_gen}
\end{algorithm}


==> backend_support.tex <==
\section{Backend Support}

\par
Generated GraphZero schedules contain only set difference and intersection operations, optionally with bounds, making the interface straightforward to implement for arbitrary backends. GraphZero includes backend implementations for both CPU and GPU, to demonstrate feasibility on varied architectures with dramatically different performance characteristics.

\par
In addition to the set operators, the backend must also implement work assignment to divide the provided graph to parallel workers. On CPU, one thread is spawned per physical core and OpenMP’s internal implementation for parallelization of a for loop assigns vertices to workers. In the GPU implementation, the backend heuristically attempts to first populate the entire GPU with workers and statically assigns a small group of vertices for each worker to execute. Once the entire GPU has been populated with workers, the backend begins to overprovision the GPU by launching additional workers. The GPU’s threadblock scheduler is used to dynamically load balance the execution of the graph for overprovisioned execution.

\subsection{Operator Implementation}

\par
Two common choices for implementing the set intersection and difference algorithms are binary search [Cite Tricore] and linear scan [Cite something?]. In a traditional linear scan implementation, each list starts with a pointer at its head. Depending on the result of the comparison of these two values, one of the pointer advances through its list. Once one pointer has reached the tail, the process has completed. Linear scan has algorithmic complexity of $O\left(m + n\right)$, where $m$ is the size of the larger list and $n$ the size of the smaller. In a binary search implementation, values are consumed from the smaller list and searched for in the second list, with algorithmic complexity $O\left(n \log m)\right)$.

\par
Based on the difference in algorithmic complexity of these two operators, there are distinct classes of intersections where linear scan should outperform binary search and vice versa. To examine this in practice, implementations of both these algorithms were implemented for both backends. To parallelize the operators on GPU, one of the lists is parallelized by striding threads and enforcing a barrier between iterations. This ensures that set instantiation maintains the original sorted ordering of vertices. The GPU implementation also prefetches the first five steps of a binary search and stores both the values and the indices of those values in shared memory.

\par
In practice however, these algorithms are sensitive to the implemented hardware. On CPU, the more regular access pattern of linear scan allows hardware prefetchers to more efficiently populate caches and results in better performance on all tested graphs. On GPU, the opposite occurred. The workload parallelization strategy provides greater benefits for binary search while also reaping the benefits of the local cache. Furthermore, introducing dynamic algorithm selection increased register file pressure [add reference to that section] on the GPU such that any potential performance gains were far outweighed by the cost of lower occupancy.
\par
As a result, schedules compiled with the CPU backend always use a linear scan implementation, while the GPU uses binary search.

\subsection{Memory Management}

For patterns larger than three vertices, it is necessary to explicitly instantiate the output of the previous set operation. Maximum dynamic memory consumption is positively correlated to the depth of the pattern and the number of patterns concurrently searched for while directly proportional to the number of task workers active at a given time. On CPU, each worker can feasibly allocate multiple gigabytes of memory simultaneously. As a result, when a set needs to be instantiated a buffer equal in size to the degree of the maximum degree vertex is requested and the vertex set is instantiated within that list. While space inefficient, this behavior ensures there are no indirect memory accesses at a very low execution overhead.

\par
However, the GPU frequently has 10-50x more workers actively running with an allocation space an order of magnitude smaller. Using the CPU allocation algorithm on GPU would preclude running all but the smallest graphs on non-trivial schedules. As a result, the GPU backend uses a paged memory manager to maximize memory usage efficiency while still maintaining compatibility with single-pass, zero intermediate set construction algorithms. As the backend constructs a set, the memory manager receives write requests. The memory manager buffers these requests in shared memory before attempting to write them to an allocated page. If the write page faults, an additional page is allocated and the spill is written to the additional page. In the case that a vertex set has spilled onto a second page, the memory manager will walk the page table to return the correct pointers for accesses.

\par
Rather than manage a set of pages for each instantiated vertex set, the backend relies on a guarantee provided by the GraphZero compiler that no instantiated vertex set will have a longer lifetime than any derived vertex sets. This enables the worker to treat the memory buffer for the instantiated sets as a single stack.

\subsection{GPU Occupancy}

\par
The GPU backend takes additional precautions to balance occupancy and worker performance. Unlike on CPU where the number of registers consumed by a program is architecturally defined, the compiler will allocate up to 255 registers per thread. Since a streaming multiprocessor has a fixed number of registers (65,536 on most modern NVIDIA architectures), register allocation is the primary constraint for the number of active workers for non-trivial schedules. The GPU backend iteratively compiles the kernel, increasing the number of allocated registers, until the thread is forced to use the maximum 255 or does not spill any registers onto the local stack.

%GraphZero generates code that only uses ?? distinct operations. 

%We choose to support both CPU and GPU as they represent two dramatically difference architectures.

%We implement two versions for each set operations. Why? Algorithm complexity. Describe the two algorithms and the optimizations for GPUs. Mention the use of bounded. Mention the different work group sizes for load balance. Make sure that you mention we have two version for each operation on both CPUs and GPUs. We may run some experiments with both versions on size-3 patterns.

%We have different memory management strategies for CPU and GPU. Explain them separately. The GPU-side memory management is particularly interesting. 



==> fast_schedule_generation/complexity_of_schedule.tex <==
\subsection{Complexity analysis}
\label{sec:complex_ana}
For this section, we analyze the complexity of our system and Automine. We define a few terms to make explaining the complexity easier
Let $M$ be the multiplicity, $N$ the number of vertices in the pattern, $E$ the number of edges, and $D$ the number of distinct valid schedules. Note that there are $DM$ valid schedules if you allow identical ones.


Automine required $O(E N!)$ time to check if two schedules were equivalent, and $\Theta(E)$ to check if one schedule is valid.
Automine checked for schedule equivalence by iterating through all permutations of the labels of a schedule and checking if any were equivalent to the other schedule, where schedules were modeled as colored complete acyclic tournaments. This is $\Theta(N!E)$ whenever they are unequal, and expected to take $N!E/2$ to find the exact permutation that makes them equal.
The method Automine used to eliminate redundant schedules was to, as valid schedules are found, check if the schedule is equivalent to one already found.
The amount of time Automine spends generating and checking all schedules for validity is $\Theta(N! E)$. 
The number of times Automine checks if a schedule is equivalent to one already found is at least $D/2$ for more than half of the valid schedules, and is at most $D$. 
Therefore, the total number of times Automine has to check equivalence of schedules is $\Theta(D^2M)$, since there are $DM$ valid schedules. To compile each of the schedules and approximate their complexity, Automine only requires $O(N^3)$ time per schedule, for a total of $O(N^3D)$. Thus, Automine requires $\Theta(N!ED^2M)$ expected time to compile a pattern. 

On our system, the complexity analysis becomes quite a bit more complicated, so we will only establish an upper bound. Our algorithm for generating all automorphisms is $O(N!E)$. Each procedure call necessarily produces at least one valid schedule, so there are $O(DN)$ procedure calls. Each of the procedure calls take $O(MN)$ time outside of their inner calls, and $O(E)$ time to generate schedules when a schedule is generated, so the algorithm is definitely  $O(DMN^2 + N!E + DE)$. 
% This is a very conservative upper bound
% Joke: Omega(DMV) is still infinite, right?

==> unused_atm/theorem_1_proof_new.tex <==
\begin{proof}
The simplest way to understand this is that after each step, there are $|Aut|$ remaining total orderings of the schedule vertices which satisfy the binary relations.
Each step removes all the automorphisms that change a given vertex, and leave only the ones that do not. 
After each vertex is fully processed, any total ordering that does not break the binary relations added so far, when applying a member of $Aut$ to it, will still not break the binary restrictions.
This is due to the fact that the vertices moved under members of $Aut$ that have restrictions applied on them will have the same restrictions if there is a mapping between them, and no restrictions between them.
\begin{lemma}
Automorphisms remaining in $Aut$ maintain validitiy under the binary relations
\end{lemma}
\begin{proof}

\end{proof}
\begin{lemma}
There is at least
\end{lemma}
\begin{proof}

\end{proof}
\end{proof}

==> unused_atm/theorem_1_proof_old_v2.tex <==
\begin{proof} This proof is split into two components. The first shows that at most one mapping exists that follows the ordering. The second shows that any instance that matches a mapping has at least one mapping that follows the restrictions.

To prove that at most one mapping exists, we perform a proof by contradiction.
Assume two distinct mappings, $M_1$ and $M_2$.
Then, $M_1$ and $M_2$ must differ in at least one vertex.
Let the first vertex in which they differ be $d$.
Then, there is an automorphism that doesn't change any of the vertices of $S$ which come before $d$, which maps $M_1$ to $M_2$. There is therefore an automorphism $A$ such that $M_1(A(x))= M_2(x)$.
Note that $M_2(d) \neq M_1(d)$, so $M_2(d) = M_1(A(d))< M_1(d)$ is a restriction that is satisfied.
However, note that this symmetrically, we also have $M_1(d) < M_2(d)$.
These two form a contradiction, so there cannot be two distinct mappings that both obey the partial orderings. This concludes the proof that at most one is achieved.

To see that there is at least one mapping that matches the ordering, note that we can satisfy each of the partial ordering restrictions in order by performing an automorphism to bring the maximum into the desired location at each step. The following Lemma is needed to prove that this automorphism wouldn't change any relations
\begin{lemma}
Any automorphism $A$ which doesn't move $S[i]$ for $i<k$ do not change the set of binary relations $(S[a],S[b])$ where $a<k$, if we apply the automorphism to each binary relation $(X,Y)$ to become $(A(X),A(Y))$, over all automorphisms. As a consequence, applying such an automorphism does not break the relations.
\end{lemma}
\begin{proof}
First, for any $b<k$, the binary relations do not move, so they are automatically satisfied.
Now, consider $(S[a],S[b])$ as a binary relation. 
Then, there exists an automorphism that doesn't move $S[j]$ for $j<a$ that maps $S[a]$ to $S[b]$.
There is then an automorphism which maps $S[a]$ to $A(S[b])$ which doesn't move $S[j]$ for $j<a$, which is the composition of those two automorphisms.
Hence $(S[a],A(S[b]))$ is a binary relation in the original set. 
Therefore, the set of binary relations after the automorphism is a subset of the binary relations before the automorphism. 
Then, symmetrically, since the automorphism is invertible, the before must be a subset of the after. 
Hence, the set of relations is the same before and after the automorphism is applied.
\end{proof}

That is, after each vertex is processed, there is still at least one mapping satisfying all of the relations. 
This is trivial before there are any relations. 
Consider a mapping $X$ that satisfies all relations generated before vertex $S[i]$ is processed.
Then, there is a maximum value among the $M(S[k])$ for which the binary relation $(S[i],S[k])$ is applied. Say this maximum occurs at $z$. 
Applying an automorphism that maps this $S[z]$ to $S[i]$ that does not change $S[j]$ for $j<i$, results in a mapping that satisfies all binary relations.
The lemma proves it satisfies the binary relations generated before vertex $S[i]$ is processed. 
In addition, it satisfies the binary relations generated while processing vertex $S[i]$, as the equivalence class of $S[i]$ under the automorphism does not change.
\end{proof}
